mvn2vec: Preservation and Collaboration in Multi-View Network Embedding

Multi-view networks are broadly present in real-world applications. In the meantime, network embedding has emerged as an effective representation learning approach for networked data. Therefore, we are motivated to study the problem of multi-view network embedding with a focus on the optimization objectives that are specific and important in embedding this type of network. In our practice of embedding real-world multi-view networks, we explicitly identify two such objectives, which we refer to as preservation and collaboration. The in-depth analysis of these two objectives is discussed throughout this paper. In addition, the mvn2vec algorithms are proposed to (i) study how varied extent of preservation and collaboration can impact embedding learning and (ii) explore the feasibility of achieving better embedding quality by modeling them simultaneously. With experiments on a series of synthetic datasets, a large-scale internal Snapchat dataset, and two public datasets, we confirm the validity and importance of preservation and collaboration as two objectives for multi-view network embedding. These experiments further demonstrate that better embedding can be obtained by simultaneously modeling the two objectives, while not over-complicating the model or requiring additional supervision. The code and the processed datasets are available at http://yushi2.web.engr.illinois.edu/.

==> Makefile <==
TARGET = mvn2vec_ieee

pdf:
	pdflatex $(TARGET) && bibtex $(TARGET) && pdflatex $(TARGET) && \
	pdflatex $(TARGET)
	open $(TARGET).pdf
	rm -f *.aux *.log *.blg *.bbl *~ *.dvi *.out *.nav *.snm *.toc *.brf *.backup $(TARGETS)


==> bio.tex <==
%!TEX root = grace.tex
\begin{IEEEbiography}[{\includegraphics[width=1in,
height=1.25in,clip,keepaspectratio]{figures/yu.jpg}}]{Yu Shi}
 is a PhD Candidate in Computer Science advised by Jiawei Han at University of Illinois at Urbana-Champaign. 
He received his bachelor's degree from the Hua Loo-Keng Talent Program in Mathematics at University of Science and Technology of China in 2014.
His research interest lies in data mining and machine learning with a focus on interpreting and modeling typed network data.
He has published in top conferences such as KDD, ICDM, SDM, and ISMB.
\end{IEEEbiography}

\begin{IEEEbiography}[{\includegraphics[width=1in,
height=1.25in,clip,keepaspectratio]{figures/fangqiu.jpg}}]{Fangqiu Han}
is a software engineer at Snap Inc. His work mainly focuses on user profiling and user understanding and their applications in various of recommendation and information retrieval systems. He received his Ph.D. in Computer Science from University of California, Santa Barbara.
\end{IEEEbiography}

\begin{IEEEbiography}[{\includegraphics[width=1in,
height=1.25in,clip,keepaspectratio]{figures/xinwei.png}}]{Xinwei He}
is senior undergraduate student major in Mathematics and Computer Science at University of Illinois Urbana Champaign. 
He is a James Scholar Student and is currently an undergraduate research assistant in professor Jiawei Han’s Data Mining Group. 
His research interests lie in information network analysis and data mining.
\end{IEEEbiography}

\begin{IEEEbiography}[{\includegraphics[width=1in,
height=1.25in,clip,keepaspectratio]{figures/xinran.png}}]{Xinran He}
is a software engineer at Snap Inc. He received his Ph.D. in Computer Science from University of Southern California. His research interests lie in social network analysis and social media analysis with a special focus on diffusion process. 
\end{IEEEbiography}

\begin{IEEEbiography}[{\includegraphics[width=1in,
height=1.25in,clip,keepaspectratio]{figures/carl.jpg}}]{Carl Yang}
is a PhD Candidate with Jiawei Han in Computer Science at University of Illinois, Urbana Champaign. He received his B.Eng. in Computer Science at Zhejiang University under Xiaofei He in 2014. In his research, he develops data-driven techniques and neural architectures for learning with complex heterogeneous data. Carl's research results have been published in top conferences like KDD, WWW, ICDE, ECML-PKDD, ICDM and ICML.
\end{IEEEbiography}

\begin{IEEEbiography}[{\includegraphics[width=1in,
height=1.25in,clip,keepaspectratio]{figures/roger.jpg}}]{Roger Jie Luo}
is an engineering and research manager at Snap Research, where he leads the R\&D efforts of multiple recommendation, discovery and search products. Before joining Snap, Roger was a senior research manager at Yahoo! Labs, Silicon Valley. At Yahoo!, he led the efforts to improve the ranking of aggregated search results (web, news, movies, local, shopping etc.) on the Yahoo! search result page and on
understanding the users' intents given a query. Roger obtained his PhD in Computer Science from Swiss Federal Institutes of Technology in Lausanne (EPFL) in 2011. He is broadly interested in different fields of artificial intelligence, and his research focused on web search, machine learning, recommendation systems, data mining, information retrieval, and multimedia information processing. He has published more than 30 papers in top-tier conferences and journals, including KDD, WWW, WSDM, SIGIR, NIPS, ICML, ICCV, CVPR, ICDM, CIKM, JMLR, TWEB. He is the recipient of 2016 WSDM Best Paper Award.  
\end{IEEEbiography}

%\vspace{-50pt}
\begin{IEEEbiography}[{\includegraphics[width=1in,
height=1.25in,clip,keepaspectratio]{figures/jiawei.jpg}}]{Jiawei Han}
is Abel Bliss Professor in the Department of Computer Science at University of Illinois at Urbana-Champaign. He received his Ph.D. in Computer Sciences at University of Wisconsin in 1985. He worked as assistant professor in Northwestern University in 1986-1987 and as assistant, associate, full and university chair professor in Simon Fraser University in 1987-2001 before joining UIUC in 2001. He has been researching into data mining, information network analysis, and database systems, and their various applications, with over 600 publications. He served as the founding Editor-in-Chief of ACM Transactions on Knowledge Discovery from Data (TKDD) (2007-2012). Jiawei has received ACM SIGKDD Innovation Award (2004), IEEE Computer Society Technical Achievement Award (2005), IEEE Computer Society W. Wallace McDowell Award (2009), Daniel C. Drucker Eminent Faculty Award at UIUC (2011), and Excellence in Graduate and Professional Teaching Award at UIUC (2012). He is a Fellow of ACM and a Fellow of IEEE. His co-authored textbook "Data Mining: Concepts and Techniques" (Morgan Kaufmann) has been adopted popularly as a textbook worldwide.
\end{IEEEbiography}
